The Adapter-Bot: All-In-One Controllable Conversational Model

Considerable progress has been made towards conversational models that generate coherent and fluent responses by training large language models on large dialogue datasets. These models have little or no control of the generated responses and miss two important features: continuous dialogue skills integration and seamlessly leveraging diverse knowledge sources. In this paper, we propose the Adapter-Bot, a dialogue model that uses a fixed backbone conversational model such as DialGPT (Zhang et al., 2019) and triggers on-demand dialogue skills (e.g., emphatic response, weather information, movie recommendation) via different adapters (Houlsby et al., 2019). Each adapter can be trained independently, thus allowing a continual integration of skills without retraining the entire model. Depending on the skills, the model is able to process multiple knowledge types, such as text, tables, and graphs, in a seamless manner. The dialogue skills can be triggered automatically via a dialogue manager, or manually, thus allowing high-level control of the generated responses. At the current stage, we have implemented 12 response styles (e.g., positive, negative etc.), 8 goal-oriented skills (e.g. weather information, movie recommendation, etc.), and personalized and emphatic responses. We evaluate our model using automatic evaluation by comparing it with existing state-of-the-art conversational models, and we have released an interactive system at adapter.bot.ust.hk.

==> img.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,1201); %set diagram left start at 0, and has height of 1201

%Rounded Rect [id:dp5325576060041444] 
\draw  [fill={rgb, 255:red, 243; green, 239; blue, 239 }  ,fill opacity=1 ] (340.2,738.85) .. controls (340.2,733.36) and (344.66,728.9) .. (350.15,728.9) -- (537.72,728.9) .. controls (543.21,728.9) and (547.67,733.36) .. (547.67,738.85) -- (547.67,819.3) .. controls (547.67,824.79) and (543.21,829.25) .. (537.72,829.25) -- (350.15,829.25) .. controls (344.66,829.25) and (340.2,824.79) .. (340.2,819.3) -- cycle ;
%Rounded Rect [id:dp5187225242210429] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (351.08,756.17) .. controls (351.08,753.96) and (352.87,752.17) .. (355.08,752.17) -- (377.08,752.17) .. controls (379.29,752.17) and (381.08,753.96) .. (381.08,756.17) -- (381.08,768.17) .. controls (381.08,770.38) and (379.29,772.17) .. (377.08,772.17) -- (355.08,772.17) .. controls (352.87,772.17) and (351.08,770.38) .. (351.08,768.17) -- cycle ;
%Rounded Rect [id:dp3142253715514356] 
\draw  [fill={rgb, 255:red, 136; green, 147; blue, 227 }  ,fill opacity=0.63 ] (381.08,756.17) .. controls (381.08,753.96) and (382.87,752.17) .. (385.08,752.17) -- (407.08,752.17) .. controls (409.29,752.17) and (411.08,753.96) .. (411.08,756.17) -- (411.08,768.17) .. controls (411.08,770.38) and (409.29,772.17) .. (407.08,772.17) -- (385.08,772.17) .. controls (382.87,772.17) and (381.08,770.38) .. (381.08,768.17) -- cycle ;
%Rounded Rect [id:dp7765741434233697] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (443.48,756.17) .. controls (443.48,753.96) and (445.27,752.17) .. (447.48,752.17) -- (469.48,752.17) .. controls (471.69,752.17) and (473.48,753.96) .. (473.48,756.17) -- (473.48,768.17) .. controls (473.48,770.38) and (471.69,772.17) .. (469.48,772.17) -- (447.48,772.17) .. controls (445.27,772.17) and (443.48,770.38) .. (443.48,768.17) -- cycle ;
%Rounded Rect [id:dp13223275141860413] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (504.08,756.17) .. controls (504.08,753.96) and (505.87,752.17) .. (508.08,752.17) -- (530.08,752.17) .. controls (532.29,752.17) and (534.08,753.96) .. (534.08,756.17) -- (534.08,768.17) .. controls (534.08,770.38) and (532.29,772.17) .. (530.08,772.17) -- (508.08,772.17) .. controls (505.87,772.17) and (504.08,770.38) .. (504.08,768.17) -- cycle ;
%Rounded Rect [id:dp43402952330403255] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (412.48,756.17) .. controls (412.48,753.96) and (414.27,752.17) .. (416.48,752.17) -- (438.48,752.17) .. controls (440.69,752.17) and (442.48,753.96) .. (442.48,756.17) -- (442.48,768.17) .. controls (442.48,770.38) and (440.69,772.17) .. (438.48,772.17) -- (416.48,772.17) .. controls (414.27,772.17) and (412.48,770.38) .. (412.48,768.17) -- cycle ;
%Straight Lines [id:da4879777665095544] 
\draw    (442,800.75) -- (408.63,776.99) ;
\draw [shift={(407,775.83)}, rotate = 395.45] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5215024194535138] 
\draw    (333.8,888.1) -- (369.37,862.66) ;
\draw [shift={(371,861.5)}, rotate = 504.43] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp9347917416168812] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.6 ] (348.6,805.96) .. controls (348.6,803.81) and (350.34,802.08) .. (352.48,802.08) -- (535.92,802.08) .. controls (538.06,802.08) and (539.8,803.81) .. (539.8,805.96) -- (539.8,817.6) .. controls (539.8,819.74) and (538.06,821.48) .. (535.92,821.48) -- (352.48,821.48) .. controls (350.34,821.48) and (348.6,819.74) .. (348.6,817.6) -- cycle ;
%Straight Lines [id:da23073081487777358] 
\draw    (504.2,703.9) -- (504.2,686.5) ;
\draw [shift={(504.2,684.5)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp47155866793746637] 
\draw   (268.67,891.83) .. controls (268.67,888.79) and (271.13,886.32) .. (274.18,886.32) -- (290.7,886.32) .. controls (293.75,886.32) and (296.21,888.79) .. (296.21,891.83) -- (296.21,916.26) .. controls (296.21,919.3) and (293.75,921.77) .. (290.7,921.77) -- (274.18,921.77) .. controls (271.13,921.77) and (268.67,919.3) .. (268.67,916.26) -- cycle ;
%Straight Lines [id:da061439298418706434] 
\draw [line width=0.75]    (273.09,893.55) -- (289.97,893.55) ;
%Straight Lines [id:da44250560099745173] 
\draw [line width=0.75]    (274.09,898.25) -- (288.05,898.25) ;
%Straight Lines [id:da07365350991446329] 
\draw [line width=0.75]    (274.09,902.95) -- (289.67,902.95) ;
%Straight Lines [id:da3120908944255891] 
\draw [line width=0.75]    (274.09,907.66) -- (283.83,907.66) ;
%Straight Lines [id:da5005997256824322] 
\draw [line width=0.75]    (274.09,912.36) -- (288.05,912.36) ;
%Straight Lines [id:da021456097595089485] 
\draw [line width=0.75]    (274.09,917.06) -- (289.67,917.06) ;
%Straight Lines [id:da7928619397131846] 
\draw [line width=0.75]    (304.76,901.08) -- (332.1,901.15) ;
%Straight Lines [id:da3599365185898049] 
\draw [line width=0.75]    (304.69,893.75) -- (304.69,916.22) ;
%Straight Lines [id:da654516362272074] 
\draw [line width=0.75]    (313.78,893.75) -- (313.78,916.22) ;
%Straight Lines [id:da3493791384866711] 
\draw [line width=0.75]    (322.86,893.75) -- (322.86,916.22) ;
%Shape: Ellipse [id:dp41343147640931033] 
\draw   (345.16,894.92) .. controls (345.6,893.18) and (347.31,892.13) .. (348.98,892.55) .. controls (350.66,892.98) and (351.66,894.72) .. (351.22,896.45) .. controls (350.78,898.18) and (349.06,899.24) .. (347.39,898.82) .. controls (345.72,898.39) and (344.72,896.65) .. (345.16,894.92) -- cycle ;
%Shape: Ellipse [id:dp6345235793095796] 
\draw   (356.06,907.39) .. controls (356.5,905.66) and (358.21,904.6) .. (359.88,905.02) .. controls (361.55,905.45) and (362.55,907.19) .. (362.11,908.92) .. controls (361.67,910.65) and (359.96,911.71) .. (358.29,911.29) .. controls (356.62,910.86) and (355.62,909.12) .. (356.06,907.39) -- cycle ;
%Shape: Ellipse [id:dp1893652658270497] 
\draw   (339.61,913.18) .. controls (340.05,911.45) and (341.76,910.39) .. (343.43,910.82) .. controls (345.11,911.24) and (346.1,912.99) .. (345.67,914.72) .. controls (345.23,916.45) and (343.51,917.51) .. (341.84,917.08) .. controls (340.17,916.66) and (339.17,914.91) .. (339.61,913.18) -- cycle ;
%Straight Lines [id:da26843355162845084] 
\draw    (344.03,910.9) -- (347.39,898.82) ;
%Straight Lines [id:da9901545689077496] 
\draw    (346.46,912.6) -- (356.31,909.71) ;
%Rounded Rect [id:dp5696529556015284] 
\draw  [fill={rgb, 255:red, 254; green, 145; blue, 150 }  ,fill opacity=1 ] (338.2,836.96) .. controls (338.2,834.81) and (339.94,833.08) .. (342.08,833.08) -- (404.45,833.08) .. controls (406.6,833.08) and (408.33,834.81) .. (408.33,836.96) -- (408.33,848.6) .. controls (408.33,850.74) and (406.6,852.48) .. (404.45,852.48) -- (342.08,852.48) .. controls (339.94,852.48) and (338.2,850.74) .. (338.2,848.6) -- cycle ;
%Rounded Rect [id:dp06295975470204174] 
\draw  [fill={rgb, 255:red, 254; green, 234; blue, 161 }  ,fill opacity=1 ] (408.2,836.96) .. controls (408.2,834.81) and (409.94,833.08) .. (412.08,833.08) -- (474.45,833.08) .. controls (476.6,833.08) and (478.33,834.81) .. (478.33,836.96) -- (478.33,848.6) .. controls (478.33,850.74) and (476.6,852.48) .. (474.45,852.48) -- (412.08,852.48) .. controls (409.94,852.48) and (408.2,850.74) .. (408.2,848.6) -- cycle ;
%Rounded Rect [id:dp8080361191788996] 
\draw  [fill={rgb, 255:red, 148; green, 222; blue, 192 }  ,fill opacity=1 ] (478.2,836.96) .. controls (478.2,834.81) and (479.94,833.08) .. (482.08,833.08) -- (544.45,833.08) .. controls (546.6,833.08) and (548.33,834.81) .. (548.33,836.96) -- (548.33,848.6) .. controls (548.33,850.74) and (546.6,852.48) .. (544.45,852.48) -- (482.08,852.48) .. controls (479.94,852.48) and (478.2,850.74) .. (478.2,848.6) -- cycle ;
%Straight Lines [id:da06331394377083388] 
\draw    (443,890.9) -- (443,866.17) ;
\draw [shift={(443,864.17)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da18899878293502104] 
\draw [line width=0.75]    (331.95,893.75) -- (331.95,916.22) ;
%Straight Lines [id:da9304789005838785] 
\draw    (553,888.1) -- (519.25,862.06) ;
\draw [shift={(517.67,860.83)}, rotate = 397.65999999999997] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp9123732177703718] 
\draw  [fill={rgb, 255:red, 148; green, 222; blue, 192 }  ,fill opacity=1 ] (468.2,710.96) .. controls (468.2,708.81) and (469.94,707.08) .. (472.08,707.08) -- (534.45,707.08) .. controls (536.6,707.08) and (538.33,708.81) .. (538.33,710.96) -- (538.33,722.6) .. controls (538.33,724.74) and (536.6,726.48) .. (534.45,726.48) -- (472.08,726.48) .. controls (469.94,726.48) and (468.2,724.74) .. (468.2,722.6) -- cycle ;
%Rounded Rect [id:dp9921689902655273] 
\draw  [fill={rgb, 255:red, 254; green, 234; blue, 161 }  ,fill opacity=1 ] (558.2,827.96) .. controls (558.2,825.81) and (559.94,824.08) .. (562.08,824.08) -- (624.45,824.08) .. controls (626.6,824.08) and (628.33,825.81) .. (628.33,827.96) -- (628.33,839.6) .. controls (628.33,841.74) and (626.6,843.48) .. (624.45,843.48) -- (562.08,843.48) .. controls (559.94,843.48) and (558.2,841.74) .. (558.2,839.6) -- cycle ;
%Rounded Rect [id:dp12254102457874616] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.6 ] (558.6,805.96) .. controls (558.6,803.81) and (560.34,802.08) .. (562.48,802.08) -- (623.79,802.08) .. controls (625.93,802.08) and (627.67,803.81) .. (627.67,805.96) -- (627.67,817.6) .. controls (627.67,819.74) and (625.93,821.48) .. (623.79,821.48) -- (562.48,821.48) .. controls (560.34,821.48) and (558.6,819.74) .. (558.6,817.6) -- cycle ;
%Curve Lines [id:da8705688538349097] 
\draw    (593.2,801.8) .. controls (550.61,766.18) and (469.89,786.46) .. (452.96,789.76) ;
\draw [shift={(451,790.1)}, rotate = 351.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da8622422396817941] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (431.2,792.47) .. controls (447.8,784.9) and (450.6,793.7) .. (451,802.1) ;
%Straight Lines [id:da6624661941451211] 
\draw [line width=0.75]    (304.76,906.08) -- (332.5,905.88) ;
%Straight Lines [id:da8368172068180149] 
\draw [line width=0.75]    (304.76,911.08) -- (332.1,911.15) ;
%Straight Lines [id:da025425403280846526] 
\draw [line width=0.75]    (304.76,916.08) -- (332.1,916.15) ;
%Straight Lines [id:da061249777667051086] 
\draw [line width=0.75]    (304.76,894.08) -- (332.1,894.15) ;

% Text Node
\draw (445.93,898.84) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont Hi, how are you today?}}};
% Text Node
\draw (366.08,762.17) node   [align=left] {{\scriptsize {\fontfamily{pcr}\selectfont  }{\fontfamily{pcr}\selectfont WoW}}};
% Text Node
\draw (396.08,762.17) node   [align=left] {{\scriptsize {\fontfamily{pcr}\selectfont  \ POS }}};
% Text Node
\draw (458.48,762.17) node   [align=left] {{\scriptsize {\fontfamily{pcr}\selectfont  PER}}};
% Text Node
\draw (519.08,762.17) node   [align=left] {{\scriptsize {\fontfamily{pcr}\selectfont EMO}}};
% Text Node
\draw (427.48,762.17) node   [align=left] {{\scriptsize {\fontfamily{pcr}\selectfont NEG}}};
% Text Node
\draw (314.87,778.57) node   [align=left] {$\displaystyle \mathnormal{N\times }$};
% Text Node
\draw (443.43,739.79) node  [font=\footnotesize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont Adapter Layers}}};
% Text Node
\draw (444.2,809.38) node   [align=left] {\begin{minipage}[lt]{58.416216000000006pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize {\fontfamily{pcr}\selectfont DialGPT Layer}}
\end{center}

\end{minipage}};
% Text Node
\draw (474,746) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \dotsc $};
% Text Node
\draw (502.8,671.78) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont I am good, thanks}}};
% Text Node
\draw (373.27,842.78) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont Meta}}};
% Text Node
\draw (443.27,842.78) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont History}}};
% Text Node
\draw (513.27,842.78) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont Reply}}};
% Text Node
\draw (584.93,897.84) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont [SOS] I am good,}}};
% Text Node
\draw (503.27,716.78) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont Reply}}};
% Text Node
\draw (593.27,833.78) node  [font=\normalsize] [align=left] {{\footnotesize {\fontfamily{pcr}\selectfont History}}};
% Text Node
\draw (593.13,811.78) node   [align=left] {\begin{minipage}[lt]{19.858108pt}\setlength\topsep{0pt}
\begin{center}
{\footnotesize {\fontfamily{pcr}\selectfont BERT}}
\end{center}

\end{minipage}};


\end{tikzpicture}

